Learning High-Dimensional Markov Forest Distributions: Analysis of Error Rates

The problem of learning forest-structured discrete graphical models from i.i.d. samples is considered. An algorithm based on pruning of the Chow-Liu tree through adaptive thresholding is proposed. It is shown that this algorithm is both structurally consistent and risk consistent and the error probability of structure learning decays faster than any polynomial in the number of samples under fixed model size. For the high-dimensional scenario where the size of the model d and the number of edges k scale with the number of samples n, sufficient conditions on (n,d,k) are given for the algorithm to satisfy structural and risk consistencies. In addition, the extremal structures for learning are identified; we prove that the independent (resp. tree) model is the hardest (resp. easiest) to learn using the proposed algorithm in terms of error rates for structure learning.

==> cor_param_prf.tex <==
\begin{proof}
If the dimension $d=o(\exp(n\delta))$, then the  upper bound in \eqref{eqn:abovelemma}  is asymptotically majorized by $\poly(n) o(\exp(n\delta))\exp(-n\delta)$.  Thus the probability tends to zero as $n\to\infty$. 
\end{proof}


==> preamble.tex <==
\usepackage[mathscr]{eucal}
\usepackage[cmex10]{amsmath}
\usepackage{epsfig,epsf,psfrag,amssymb,amsfonts,latexsym,url,amsmath,graphicx,bm,cite, xcolor,url}
\usepackage[caption=false]{subfig}%,font=footnotesize
\usepackage{fixltx2e}%ordering of single and double column floats
%\usepackage{array}%array and tabular environments
%\usepackage{mdwmath,mdwtab}%format equations and tables: problems with \Bigl(
%\usepackage{cases}%[subnum]
%\usepackage{setspace}
\usepackage{verbatim}
\usepackage{bm}
\usepackage{latexsym, amssymb, amsmath}
%\usepackage{bbold}
%\usepackage{setspace}
%\usepackage{algpseudocode}%

%\allowdisplaybreaks[1]

\def\beq{\vskip .1cm \begin{equation}}
\def\eeq{\end{equation} \vskip .1cm \noindent}
\def\beqn{\vskip .1cm \begin{eqnarray}}
\def\eeqn{\end{eqnarray} \vskip .1cm \noindent}
\def\beqnn{\vskip .01cm \begin{eqnarray*}}
\def\eeqnn{\end{eqnarray*} \vskip .01cm \noindent}
\def\bfp{{\mathbf p}}
\def\bfq{{\mathbf q}}
\def\Pbb{{\mathbb P}}
\def\Ebb{{\mathbb E}}
\def\nn{\nonumber}
\def\defeq{{:=}}

 
\def\Comment{{\bf comment\_anima }} 
\def\VComment{{\bf comment\_Vincent }} 
\newcommand{\nbd}{\mathrm{nbd}}
%\newcommand{\PFA}{p_{\text{\scriptsize FA}}^{(n)}}
%\newcommand{\PM}{p_{\text{\scriptsize M}}^{(n)}}
\newcommand{\QGLRT}{Q^*_{\text{\scriptsize GLRT}}}
\newcommand{\mathdef}{\stackrel{\mathrm{def}}{=}}
\newcommand{\CLThres}{\mathsf{CLThres}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calF}{\mathcal{F}}
%\newcommand{\qed}{\hfill \ensuremath{\Box}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\ML}{\mathrm{ML}}
\newcommand{\eig}{\mathrm{eig}}
\newcommand{\MAP}{\mathrm{MAP}}
\newcommand{\vect}{\mathrm{vec}}
\newcommand{\pa}{\mathrm{pa}}
\newcommand{\hQ}{\widehat{Q}}
\newcommand{\hmu}{\widehat{\mu}}
\newcommand{\hT}{\widehat{T}}
\newcommand{\Pd}{P^{(d)}}
\newcommand{\Qd}{Q^{(d)}}
\newcommand{\tilPd}{\widetilde{P}^{(d)}}
\newcommand{\tilQ}{\widetilde{Q}}
\newcommand{\tilC}{\widetilde{C}}
\newcommand{\tilP}{\widetilde{P}}
\newcommand{\tilM}{\widetilde{M}}
\newcommand{\tilQd}{\widetilde{Q}^{(d)}}
\newcommand{\tilGamma}{\widetilde{\Gamma}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\frakS}{\mathfrak{S}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\hcalU}{\widehat{\mathcal{U}}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\bP}{\mathbb{P}}
%\newcommand{\glb}{g.l.b.}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bmeta}{\bm{\eta}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bdelta}{\bm{\delta}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\hp}{\widehat{p}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\hP}{\widehat{P}}
\newcommand{\hE}{\widehat{E}}
\newcommand{\he}{\widehat{e}}
\newcommand{\hk}{\widehat{k}}
\newcommand{\veps}{\varepsilon}
\newcommand{\hrho}{\widehat{\rho}}
\newcommand{\hPML}{{P}_{{\text{\tiny ML}}}}
\newcommand{\hI}{\widehat{I}}
\newcommand{\PML}{P_{\mathrm{ML}}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\hTML}{\widehat{T}_{\ML}}
\newcommand{\TML}{{T}_{\ML}}
\newcommand{\Path}{\mathrm{Path}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\tilp}{\widetilde{p}}
\newcommand{\tilJ}{\widetilde{J}}
\newcommand{\tilS}{\widetilde{S}}
\newcommand{\beps}{\bm{\epsilon}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\etal}{et al.}
\newcommand{\beye}{\mathbf{I}}
\newcommand{\hcalE}{{\calE}_{{\text{\tiny ML}}}}
\newcommand{\hPd}{\hP^{(d)}}
\newcommand{\hQd}{\hQ^{(d)}}
%\newcommand{\Sd}{S_d}
\newcommand{\hS}{\widehat{S}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\eg}{{\it e.g.}}

%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{remark}[theorem]{Remark}

%\newtheorem{definition}{Definition}
%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{example}[1][Example]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}


==> scaling_param_prf.tex <==
\begin{proof}
The proof relies on the following conditioning result, which is similar to Lemma~\ref{lem:reduction}. Recall that $\calB_n=\{\hE_k=E_P\}$ is the event that the top $k$ edges in the estimated edge set are the same as the edges in $E_P$. 
\begin{lemma} \label{lem:reduction_2}
For every $\eta>0$, there exists a $N \in\bN$ such that for all $n>N$, the following bounds hold:
\begin{align}
&(1-\eta)P^n(D(P^* \, ||\, P)>\delta |\calB_n)\le P^n(D(P^* \, ||\, P)>\delta) \nn\\
&\le P^n(D(P^* \, ||\, P)>\delta |\calB_n)+\exp(-n(K_P-\eta)). \label{eqn:boundDPstar}
\end{align}
\end{lemma}
Thus it suffices to upper and lower bound $ P^n(D(P^* \, ||\, P)>\delta |\calB_n)$  and to show that it equals $\exp(-n\delta/d)$ to first order in the exponent. To do so, we rely on the following lemma, which is a generalization of a  well known result~\cite[Ch.\ 11]{Cov06}. We defer the proof to the end of the section. 
\begin{lemma}[Divergence  Bounds]  \label{lem:dpq_bound}
Let $X,Y$ be two  random variables whose joint distribution is $P_{X,Y}\in\calP(\calX^2)$ and $|\calX|=r$. Let $(x^n, y^n)$ be $n$ independent observations of $P_{X,Y}$. Then, for every $n$,
\begin{equation}
P_{X,Y}^n(D(\hP_{X|Y}\, ||\, P_{X|Y})>\delta)\le (n+1)^{r^2} \exp(-n\delta), \label{eqn:kl_div_bound} 
\end{equation}
where $\hP_{X|Y}$ is the conditional type of $(x^n, y^n)$. Furthermore, 
\begin{equation}
\liminf_{n\to\infty} \frac{1}{n}\log P_{X,Y}^n(D(\hP_{X|Y}\, ||\, P_{X|Y})>\delta)\ge -\delta.  \label{eqn:kl_div_lower_bound} 
\end{equation}
\end{lemma}
Note that if $X$ and $Y$ are independent, the  $P_{X|Y}$ term in~\eqref{eqn:kl_div_bound}  is equal to $P_X$. This simple observation will be useful in the proof. Note also that the  bounds in~\eqref{eqn:kl_div_bound}  and~\eqref{eqn:kl_div_lower_bound}  are independent of the distribution $P_{X,Y}$. We now proceed with the proof of Theorem~\ref{thm:consisten_param}. To do so, we consider the directed representation of the tree distributions as in \eqref{eqn:tree_decomp_directed}. Conditioned on the fact that the first $k$ edges of the graph of $P^*$ are the same as those in $E_P$ (event $\calB_n$), the KL-divergence between $P^*$ and $P$ can be expressed as a sum over $d$ terms:
\begin{equation}
D(P^* \, ||\, P)=\sum_{i\in V}D(\hP_{i|\pa(i;\hE)}\, ||\, P_{i|\pa(i;E_P)}), \label{eqn:divergence_decomp}
\end{equation}
where  the parent of $i$ in $E_P$ is defined as $\pa(i;E_P):=\pa(i;\hE)$  if $(i,\pa(i;\hE))\in E_P $ and $\pa(i;E_P):=\emptyset$ otherwise. Then, the probability $P^n(D(P^* \, ||\, P)>\delta |\calB_n)$ in \eqref{eqn:boundDPstar} can be upper bounded as 
\begin{align}
 &=  P^n\left(\sum_{i\in V}D(\hP_{i|\pa(i;\hE)}\, ||\, P_{i|\pa(i;E_P)})>\delta \Big|\calB_n\right) \label{eqn:parents_decomp}\\
&= P^n\left(\frac{1}{d}\sum_{i\in V}D(\hP_{i|\pa(i;\hE)}\, ||\, P_{i|\pa(i;E_P)})>\frac{\delta}{d} \Big|\calB_n\right) \label{eqn:divide_d}\\
&\le P^n\left(\max_{i\in V} \left\{D(\hP_{i|\pa(i;\hE)}\, ||\, P_{i|\pa(i;E_P)}) \right\}>\frac{\delta}{d} \Big|\calB_n \right) \label{eqn:max_bound}\\
%&= P^n\left(\bigcup_{i\in V}  \left\{D(\hP_{i|\pa(i;\hE)}\, ||\, P_{i|\pa(i;E)}) \right\}>\frac{\delta}{d} \Big|\calB_n \right) \label{eqn:max2union}\\
&\le \sum_{i\in V} P^n\left( D(\hP_{i|\pa(i;\hE)}\, ||\, P_{i|\pa(i;E_P)})  >\frac{\delta}{d} \Big|\calB_n \right) \label{eqn:union_bound_max}\\
&\!\le\! \sum_{i\in V} \! (n+1)^{r^2} \exp\left(\!-\!n\frac{\delta}{d}\right) \!=\! d  (n+1)^{r^2} \!\exp\! \left(\!-\!n\frac{\delta}{d}\right) \label{eqn:abovelemma}
\end{align}
where Eq.~\eqref{eqn:parents_decomp} follows from the decomposition in \eqref{eqn:divergence_decomp}.  Eq.~\eqref{eqn:max_bound} follows from the fact that if the mean of $d$ positive numbers exceeds $\delta'=\delta/d$, then the maximum must necessarily exceed $\delta'$. Eq.~\eqref{eqn:union_bound_max} follows from the union bound. Eq.~\eqref{eqn:abovelemma} follows from the upper bound in Lemma~\ref{lem:dpq_bound} which also holds if $\pa(i;E_P)=\emptyset$. Note also that $|V|=d$.  Eq.~\eqref{eqn:abovelemma} and Lemma~\ref{lem:reduction_2} together complete the proof of  \eqref{eqn:param_upper} in Theorem~\ref{thm:consisten_param}. 

Now we exploit the lower bound in Lemma~\ref{lem:dpq_bound} to prove the lower bound in Theorem~\ref{thm:consisten_param}. The probability $P^n(D(P^* \, ||\, P)>\delta |\calB_n)$ in \eqref{eqn:boundDPstar} can be lower bounded by
\begin{align}
& \max_{i\in V}\,\, P^n\left(  D(\hP_{i|\pa(i;\hE)}\, ||\, P_{i|\pa(i;E_P)})  >\delta \Big|\calB_n\right) \label{eqn:lower_d} \\
&\ge  \exp(-n(\delta+\eta)), \label{eqn:lower_d_exponent}
\end{align}
where Eq.~\eqref{eqn:lower_d} follows from the decomposition in \eqref{eqn:parents_decomp} and Eq.~\eqref{eqn:lower_d_exponent} holds for every $\eta$ for sufficiently large $n$ by \eqref{eqn:kl_div_lower_bound}.  This completes the proof of \eqref{eqn:param_lower}  upon taking the normalized logarithm and $\liminf$ in $n$ and using Lemma~\ref{lem:reduction_2}.

The fact that $D(P^*\, ||\, P)=O_P(d/n)$ is a consequence of the bound in \eqref{eqn:abovelemma}. This completes the proof of Theorem~\ref{thm:consisten_param}. 
\end{proof}

\begin{proof} ({\em of Lemma~\ref{lem:dpq_bound}})
Define the $(P_{X,Y},\delta)$-conditional-typical set to be 
\begin{equation}
\calS_{P_{X,Y}}^{\delta}:= \{ (x^n,y^n)\in (\calX^2)^n:D(\hP_{X|Y}\, ||\, P_{X|Y})\le\delta\}.
\end{equation}
We now estimate the probability that a sequence is conditional-atypical, i.e., $P^n_{X,Y}((\calS_{P_{X,Y}}^{\delta})^c) $
\begin{align}
&= \sum_{Q_{X,Y}\in(\calS_{P_{X,Y}}^{\delta})^c} P^n_{X,Y}(\bbT(Q_{X,Y}))  \label{eqn:sum_type_class}\\
&\le \sum_{Q_{X,Y}\in(\calS_{P_{X,Y}}^{\delta})^c} \exp(-nD(Q_{X,Y}\, ||\, P_{X,Y})) \label{eqn:method_types_upper}\\
%&= \sum_{Q_{X,Y}\in\calP_n(\calX^2):D(Q_{X|Y}\, ||\, P_{X|Y})>\delta}  \!\!\!|!\! \exp(-n (D(Q_{X|Y}\, ||\, P_{X|Y})+ D(Q_{Y}\, ||\, P_{Y}))) \label{eqn:div_decomp} \\
&\le \sum_{Q_{X,Y}\in(\calS_{P_{X,Y}}^{\delta})^c}    \exp(-n D(Q_{X|Y}\, ||\, P_{X|Y})  ) \label{eqn:div_pos} \\
&\le \sum_{Q_{X,Y}\in(\calS_{P_{X,Y}}^{\delta})^c}  \exp(-n \delta  ) \label{eqn:delta_bound} \\
&\le (n+1)^{r^2} \exp(-n \delta  ) \label{eqn:num_types}
\end{align}
where Eq.~\eqref{eqn:method_types_upper} follows from the method of types in Lemma~\ref{lem:typeclass}. Eq.~\eqref{eqn:div_pos} follows from the chain rule and non-negativity of the relative entropy. Eq.~\eqref{eqn:delta_bound} follows from the fact that $D(Q_{X|Y}\, ||\, P_{X|Y})>\delta$ for $Q_{X,Y}\in(\calS_{P_{X,Y}}^{\delta})^c$. Finally, Eq.~\eqref{eqn:num_types} follows the fact that the number of types with denominator $n$ is bounded by  $ (n+1)^{r^2} $. This concludes the proof of \eqref{eqn:kl_div_bound} . As an aside, note that since \eqref{eqn:num_types} is summable, we can apply the   Borel-Cantelli lemma to also conclude that $D(\hP_{X|Y}\,||P_{X|Y})$ converges to zero almost surely. 

We now prove the lower bound in \eqref{eqn:kl_div_lower_bound}. First, construct a sequence of distributions  $\{Q_{X,Y}^{(n)}\in\calP_n(\calX^2)\}_{n\in\bN}$ such that $D(Q_{Y}^{(n)}||P_{Y})=0$ and $D(Q_{X|Y}^{(n)}||P_{X|Y})=\delta+n^{-1}$.     Thus, starting from \eqref{eqn:sum_type_class}, we have for every $n$,
\begin{align}
P^n_{X,Y}(  &(\calS_{P_{X,Y}}^{\delta})^c) \ge P_{X,Y}^n  ( \bbT(Q_{X,Y}^{(n)})) \\
&\ge (n+1)^{-r^2}\exp(-nD(Q_{X,Y}^{(n)}\, ||\, P_{X,Y})).
\end{align}
Taking the normalized logarithm on both sides  and the $\liminf$ yields
\begin{align}
& \liminf_{n\to\infty} \frac{1}{n}\log P^n_{X,Y}(  (\calS_{P_{X,Y}}^{\delta})^c)  \nn \\
& \ge \liminf_{n\to\infty} \!\left\{ \!-D(Q_{X|Y}^{(n)}|| P_{X|Y})\!-\! D(Q_{Y}^{(n)}|| P_{Y}) \!\right\}\!=\!-\delta.
\end{align} 
This concludes the proof of Lemma~\ref{lem:dpq_bound}.
\end{proof}
 

